Lego Sketch: A Scalable Memory-augmented Neural Network for Sketching Data Streams

Sketches, probabilistic structures for estimating item frequencies in infinite data streams with limited space, are widely used across various domains. Recent studies have shifted the focus from handcrafted sketches to neural sketches, leveraging memory-augmented neural networks (MANNs) to enhance the streaming compression capabilities and achieve better space-accuracy trade-offs.However, existing neural sketches struggle to scale across different data domains and space budgets due to inflexible MANN configurations. In this paper, we introduce a scalable MANN architecture that brings to life the {\it Lego sketch}, a novel sketch with superior scalability and accuracy. Much like assembling creations with modular Lego bricks, the Lego sketch dynamically coordinates multiple memory bricks to adapt to various space budgets and diverse data domains. Our theoretical analysis guarantees its high scalability and provides the first error bound for neural sketch. Furthermore, extensive experimental evaluations demonstrate that the Lego sketch exhibits superior space-accuracy trade-offs, outperforming existing handcrafted and neural sketches. Our code is available at https://github.com/FFY0/LegoSketch_ICML.

==> SubFiles/method.tex <==
\section{Method}
\subsection{Preliminary}
Transformer-based LLMs typically follows an autoregressive decoding manner. Given a token sequence of length $n$, denoted as $ x_{1:n} = (x_1, x_2, \ldots, x_n) $, the autoregressive model $M$ outputs the probability distribution $ p(x_{n+1})= M(x_{1:n}) $ for the next token $ x_{n+1} $. Subsequently, the next token $x_{n+1}$ is sampled from $p(x_{n+1})$ using a specific strategy (e.g., greedy, top-K, top-P [cite]). However, as the focus of this paper is not on sampling strategies, we uniformly employ the simplest and most common strategy, greedy sampling, selecting the candidate with the highest probability as the inferred token. Therefore, the process of autoregressive decoding for a token sequence $x_{n+1:n+m}$ of length $m$ one by one is described as : $x_{n+t}=\operatorname{argmax}{M(x_{1:n+t-1})} \:|\: t\in [1, m]$.
\subsection{Overview}
To accelerate decoding in a target LLM, \(M_{\text{target}}\), our approach, termed Myopia, is structured into two primary phases: draft and verification, similar to other speculative decoding processes. During the draft phase, we modify the default global attention mechanism of \(M_{\text{target}}\) to a local attention configuration. This modification enables the creation of a self-drafted model, \(M_{\text{draft}}\), which could  rapidly draft tokens for itself. In the subsequent verification phase, the original target model \(M_{\text{target}}\) directly assesses the generated drafts.

As demonstrated in Algorithm \ref{alg:frame}, given an initial input sequence \( x_{1:n} \), \( M_{\text{target}} \) first conducts a prefill computation to populate global attention KV caches for all initial tokens. Mypopia then iteratively invokes both \(M_{\text{draft}}\) and \(M_{\text{target}}\) within a Draft\&Verification paradigm to cyclically generate sequences. At each step, \(M_{\text{draft}}\) first drafts K tokens candidates. Following this, in the verification phase, \(M_{\text{target}}\) concurrently verifies all draft tokens in parallel. This cycle continues iteratively until the sequence generation concludes. By implementing this two-phase structure, Myopia accelerates the decoding process in \(M_{\text{target}}\) while ensuring that the generated sequences maintain high fidelity and coherence.


\begin{comment}
	\begin{algorithm}[H]
		\SetAlgoLined
		\KwResult{Squence X}
		\KwIn{Target LLM $M_{target}$, draft model $M_{draft}$, input sequence $x_{1:n}$, draft length $K$}
		%\KwOut{Your output variables.}
		\textbf{Prefill} the KV Cache $M_{target}(x_{1:n})$\\
		\While{Not End}{ 		
			\For{$i \leftarrow 1$ \KwTo $K$}{ \\
				x
				$L[i] \leftarrow i^2$\;
			}
		}
	\end{algorithm}

\begin{algorithm}[H]
	\SetAlgoLined
	\KwIn{Target LLM $M_{\text{target}}$, draft model $M_{\text{draft}}$, input sequence $x_{1:n}$, draft length $K$, Max generated Length T}
	
	$init length \leftarrow n$ \\
	\textbf{Prefill} the KV Cache $M_{\text{target}}(x_{1:n})$\;
	\While{$n \leq init length + T$}{
		\tcp{Autoregressive draft phase with $M_{draft}$} 			
		\For{$i \leftarrow 1$ \KwTo $K$ in sequence}{
			$\hat{x}_{n+i} \leftarrow \operatorname{argmax} M_{draft}(x_{1:n+i-1}) $
			% Assuming the operation is a placeholder, replace with actual operation
		}
		\tcp{Parrallel verification phase with $M_{target}$}
		\For{$j \leftarrow 1$ \KwTo $K$ in parrallel}{
			$x_{n+j} \leftarrow \operatorname{argmax} M_{target}(x_{1:n+j-1})$\\
			\If{$x_{n+j} = \hat{x}_{n+j}$}{ Accept $\hat{x}_{n+j}$; }
			\Else{
				Accept $x_{n+j}$ and reject all tokens after $\hat{x}_{n+j}$; \\
				break; % Exit the loop
			}
		}
		$n \leftarrow n+j$;\\
	}
	\caption{Example Algorithm with Prefill and Looping}
\end{algorithm}
\end{comment}



	
	\begin{algorithm}[H]
		\SetAlgoLined
		\DontPrintSemicolon  % Removes semicolons to save space
		\KwIn{Target LLM $M_{\text{target}}$, draft model $M_{\text{draft}}$, input token sequence $x_{1:n}$, draft length $K$,\\ max generating length $T$}
		\KwOut{Ouput token sequence $x_{n+1:n+T}$}
		$m \leftarrow n$\;
		\textbf{prefill} the KV Caches using $M_{\text{target}}(x_{1:m})$\;
		\While{$m \textless n + T$}{
			\tcp{Draft phase with $M_{draft}$} 			
			\lFor{$i \leftarrow 1$ \KwTo $K$}{
				$\hat{x}_{m+i} \leftarrow \operatorname{argmax} M_{draft}(x_{1:m};\hat{x}_{m+1:m+i-1})$ \textbf{in sequence}  
			}
			\tcp{Verification phase with $M_{target}$}
			\lFor{$i \leftarrow 1$ \KwTo $K$}{$\check{x}_{m+i} \leftarrow \operatorname{argmax} M_{target}(x_{1:m};\hat{x}_{m+1:m+i-1})$ \textbf{in parallel}}
			\tcp{Selectively accept draft tokens}
			$count \leftarrow 0$\\
			\For{$i \leftarrow 1$ \KwTo $K$}{
				\textbf{accept} ${x}_{m+i} \leftarrow \check{x}_{m+i}$ \\
				$count \leftarrow count + 1$\\
			\lIf{$\hat{x}_{m+i} != \check{x}_{m+i}$}{
					\textbf{reject} remaining tokens and \textbf{break} the loop 
				}	
			}
			$m\leftarrow m + count$; % Updating n outside of the loop to correctly continue the sequence generation
		}
		\Return{$x_{n+1:n+T}$}
		\caption{Speculative Mypoia}
		\label{alg:frame}
	\end{algorithm}
%Like other speculative decoding algorithms, our Myopia is structured into two phases: draft and verification. During each step, the draft model initially generates several token candidates. Subsequently, in the verification phase, the original LLM concurrently verifies generated sequences composed of these token candidates in parallel.

%This verification stage determines which token candidates from the draft are accepted and appended to the sequence, and which are disregarded. Specifically, the draft model $M_{draft}$ autoregressively  outputs and samples token distributions $p_{draft}(x_{n+t})$ from the input \(x_{1:n+t-1}\) $m$ times, ultimately generating the draft sequences $x_{n+1, n+m}$. Subsequently, the original LLM \(M_{\text{origin}}\) parallelly evaluates the probability of each token $p_{origin}(x_{n+t})$, and decides whether to accept or discard them based on criteria, such as the previously mentioned greedy sampling.


==> SubFiles/relatedworks.tex <==
\section{Related Works}
Data streams, characterized by a continuous sequence of data items, are pivotal in modern data processing. Their immense volume and rapid flow  pose significant challenges for not only  processing time but also space requirements.
	Real-time analysis of these streams often necessitates some probabilistic data structures,e.g. CM-sketch, bloom filter and hypterLogLog, to provide acceptable solutions within limited computational resources.
	 Traditional approaches leverage empirical knowledge of data stream distributions, such as skewness, to continually develop novel mechanisms atop these base probabilistic structures, enhancing accuracy.
	 Concurrently, some researchers have also attempted exploring deep learning to augment base probabilistic data structures. 
	  However, these advancements, whether through manual or deep learning augmentations, still depend on base handcrafted structures. 
	 Recent studies are thus exploring memory-augmented neural networks, aiming to supplant handcrafted base probabilistic structures with entirely neural base architectures. 
	 This paradigm shift promises significant accuracy improvements in certain scenarios but also introduces challenges in generalization and scalability.
	 Our paper introduces a novel neural base sketch, called Lego sketch for frequency estimation in data streams, which not only boosts accuracy but also addresses previous challenges of generalization and scalability.  
	 



	\textit{Base sketches} employ several basic hash functions and a compact matrix of counters for approximating data items frequencies in streams, varying in the strategies based on store and retrieval. 
	For example, CM-Sketch, C Sketch as the two most common base sketches use 2D arrays for compressed storage of data streams. 
	Besides, certain base sketch variants use different strategies on 2D arrays to meet  the requirements of specific scenarios.
	
	\textit{Augmented sketches}, exemplified by ASketch,Cold Filter and Elastic Sketch, build upon base Sketches by integrating extra structures for stream preprocessing to boost performance. Notably, the elastic sketch utilizes a set of voting-based counting buckets to filter high-frequency items in data streams upon a CM-sketch. This approach effectively mitigates the hash collisions between high and low-frequency items within the its core base sketch.
	
	With augmented sketches by manually capturing distributions progressing, some researchers have attempted to utilize deep learning to enhance the accuracy further.  Initially, these developments were confined to the augmented sketch category, termed neural augmented sketch. These researches employ neural networks to discern between high and low-frequency data items, aiming to mitigate conflicts through segregated processing. The representation of this methodology is the learned sketch [cite], which employs neural networks to classify high and low-frequency items. High-frequency items, as predicted, are individually tallied in designated counters, whereas low-frequency items are collectively accounted for in a base sketch. However, the underlying assumption of neural augmented sketch—that the correspondence between items and frequencies is static and that ample features are available for neural network-based classification—is often invalidated in varied real-world data streams, thereby imposing intrinsic limitations on such methodologies.
	
	
The latest Meta Sketch [cite], along with the methodologies presented in this paper, falls under the category of neural base sketch, delineating a new path that is orthogonal to all existing techniques in (neural) augmented sketches. Notably, the neural base sketches disregard the correspondence between items and their frequencies within data stream distributions, consequently expanding their application potential far beyond that of neural augmented sketch techniques. Drawing inspiration from NBF[cite], another neural base data structure in other stream field, the meta sketch pioneers the application of Memory Augmented Neural Networks(MANN) to create the first purely neural base sketch, directly embedding data items into the network's memory slots. This innovation is complemented by a self-supervised training algorithm rooted in meta-learning, equipping the model to adeptly estimate item frequencies within data streams. Empirical evidence reveals that Meta Sketch outperforms traditional Sketch techniques in scenarios of constrained memory space resources. 

follow the approach of employing meta-learning and memory neural networks to build base data structures within the neural data structure family, proposing a novel neural base sketch, called Lego sketch. Leveraging the meta-learning training strategy used in meta sketch focused on learning the skewness of distributions, we have introduced a suite of innovations. These include a novel tailored MANN architecture, a self-guided loss weighting method, and a theoretically grounded scalability strategy, effectively overcoming numerous challenges inherent in data structures solely based on neural networks. Furthermore, for the first time, we have attempted to integrate the orthogonal techniques in augmented sketches into the realm of neural base sketches. The detailed novelty contributions of the Lego sketch are summarized as follows:

==> SubFiles/structure.tex <==
\subsection{Structure}
